On the limits of agency in agent-based models

Agent-based modeling (ABM) offers powerful insights into complex systems, but its practical utility has been limited by computational constraints and simplistic agent behaviors, especially when simulating large populations. Recent advancements in large language models (LLMs) could enhance ABMs with adaptive agents, but their integration into large-scale simulations remains challenging. This work introduces a novel methodology that bridges this gap by efficiently integrating LLMs into ABMs, enabling the simulation of millions of adaptive agents. We present LLM archetypes, a technique that balances behavioral complexity with computational efficiency, allowing for nuanced agent behavior in large-scale simulations. Our analysis explores the crucial trade-off between simulation scale and individual agent expressiveness, comparing different agent architectures ranging from simple heuristic-based agents to fully adaptive LLM-powered agents. We demonstrate the real-world applicability of our approach through a case study of the COVID-19 pandemic, simulating 8.4 million agents representing New York City and capturing the intricate interplay between health behaviors and economic outcomes. Our method significantly enhances ABM capabilities for predictive and counterfactual analyses, addressing limitations of historical data in policy design. By implementing these advances in an open-source framework, we facilitate the adoption of LLM archetypes across diverse ABM applications. Our results show that LLM archetypes can markedly improve the realism and utility of large-scale ABMs while maintaining computational feasibility, opening new avenues for modeling complex societal challenges and informing data-driven policy decisions.

==> content/agent_torch.tex <==
% Scalability -> Get started quickly (Sec 1?)
% Differentiability -> Gradient-descent on sim params (Sec 4); Customize agent (Sec 4)
% Composability -> Compose with NN (Sec 6);
% Flexibility -> Debug prompts (Sec 7); Analyzer (Sec 7)

\section{AgentTorch framework}
\AQ{I think some of this can go to the appendix, we don't need that much emphasis on the framework and I would focus on the archetypes and diferentiability through them as well. So would expand the differentiability aspect here a bit more.}
%\textbf{Framework}: While the concepts introduced in this section provide a foundation for understanding ABMs, existing frameworks have limitations in terms of scalability, differentiability, and compatibility with LLM agents \AQ{we need to be careful here, differentiability is independent of LLM agents}. The utility of ABMs for practical decision-making requires recreating populations with great detail, specifying complex dynamics and interventions, and capturing the adaptability of individual behavior. Conventional ABM frameworks (e.g., Mesa, NetLogo, Agents.jl) allow for building complex environments but are slow to execute, do not support differentiable or neural computation, and are not designed to be compatible with LLM agents. Recent frameworks (e.g., Concordia) are designed for LLM agents but are primarily tailored for tabletop games and do not scale to large populations or complex intervention dynamics. To address these challenges, we introduce AgentTorch, a framework that enables the design of large-scale, adaptive ABMs with LLM agents. In the 

AgentTorch is a framework that enables the creation of ABMs with complex dynamics, adaptive individual behavior, and efficient simulation of million-size populations. The key features are:
% AgentTorch enables the simulation, calibration, and analysis of country-scale ABMs on commodity hardware.
% \AQ{@Ayush: to review this} AgentTorch is a framework that enables the simulation, calibration, and analysis of ABMs with complex environmental dynamics and million-size populations of agents with adaptive behaviour. 
\begin{itemize}
    \item \textbf{Scalability}: AgentTorch leverages vectorized computing to specify environment dynamics and interventions which enables the simulation of millions of agents on commodity hardware. For example, AgentTorch implementations of epidemiological ABMs with 60 million agents have shown improvements up to 40,000x in computational time\cite{10.5555/3545946.3598853} respect to models developed with traditional object-oriented frameworks~\cite{datseris2022agents,mesa}. With the use of archetypes (\autoref{sec:archetypes}), these gains are preserved even when using LLM-informed agents, as opposed to frameworks like Concordia~\cite{vezhnevetsGenerativeAgentbasedModeling2023a} which are limited to very small populations.
    % AgentTorch-based implementations of epidemiological ABMs with 60 milion agents have shown improvements of up to 40,000x in computational time \cite{chopraDifferentiableAgentbasedEpidemiology2023c} respect to models developed with traditional object-oriented frameworks such as Mesa[] or NetLogo[]. With the use of archetypes (\autoref{sec:archetypes}), these computational gains are preserved even when using LLM-informed agents, as opposed to frameworks like Concordia [] which are limited to very small populations. 
    \item \textbf{Differentiability}: AgentTorch provides custom utilities to build differentiable implementations of continuous and discrete environments. With the use of gradient-assisted calibration techniques, AgentTorch can calibrate large numbers of parameters to heterogeneous datasets~\cite{chopraDifferentiableAgentbasedEpidemiology2023c,chopra2024framework}. For example, unlike in torch, you can differentiate through 
    agent\_torch.bernoulli and agent\_torch.logical\_and (more details in appendix A). 
    % To our knowledge, this is the first differentiable ABM framework. 
    %AgentTorch allows for the differentiation of environment dynamics, enabling the use of gradients for calibration and sensitivity analysis. This is achieved through custom utilities for differentiating through continuous and discrete stochasticity (eg:AgentTorch.Bernoulli; AgentTorch.logical\_and produce gradients!). Differentiability also enables the composition of ABMs with neural networks to ingest heterogeneous data sources for calibration and specify arbitrarily complex dynamics.
    \item \textbf{Composability}: AgentTorch allows for the composition of ABMs with neural networks and LLMs, enabling the design of more expressive and flexible agent architectures. The differentiability of the environments ensures that these systems remain end-to-end differentiable. The framework provides APIs that integrate with generative agent frameworks such as LangChain and dspy LLM instances. See code snippets in \autoref{fig:master-figure} and \autoref{fig:code_compose}.
    
    %AgentTorch's performance efficiency and modularity enable the composition of ABMs with LLMs and neural networks, allowing for the capture of adaptive individual behavior. The framework provides a simple Python API for building ABMs and can compose with generative agent frameworks like LangChain and dspy LLM instances.
\end{itemize}

\begin{figure*}[h!]
    \includegraphics[width=0.99\textwidth]{plots/fig2_final.png}
    % \begin{subfigure}[b]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/code/agent_torch_sim.png}
    %     \label{fig:image1}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/code/agent_torch_grad.png}
    %     \label{fig:image2}
    % \end{subfigure}
    \caption{AgentTorch API for (left) archetypes to sample population-wide isolation behavior (see:\autoref{sec:benchmark_llm_agents}); (right) composing ABMs with DNNs for end-to-end optimization (see:\autoref{sec:calibration}).}
    \label{fig:code_compose}
\end{figure*}

    % (left) Code snippet for using archetypes to sample population-wide isolation behavior in NYC (used in )
    
    % to load archetypes based on the NYC population census. The isolation behaviour can then be sampled efficiently. right side: code snippet showcasing the seamless integration of AgentTorch ABMs into neural pipelines, allowing differentiation end to end for gradient-assisted calibration


\AQ{Maybe move to discussion or introduction?} AgentTorch's design is motivated by active collaborations around the world, with models currently being deployed to help mitigate a measles outbreak in New Zealand~\cite{new_zealand_tutorial}; capture the foraging behavior of migratory birds in Alaska; and analyze the dairy supply chain in the Pacific islands to safeguard against a potential H5N1 outbreak. Previously, AgentTorch models were used across multiple countries during the COVID-19 pandemic to evaluate immunization protocols~\cite{romero2021public, chopra2023using} deployed across multiple countries~\cite{lancet_retrospective, nz_news}. The project is under active development, and we refer to the GitHub repository for tutorial notebooks, videos, reference implementations, installation guides, and contribution guidelines. To familiarize with the architecture, the project website\footnote{agenttorch.github.io/AgentTorch} includes hands-on notebooks to build a new environment and execute simulations using an existing environment. We also provide code snippets in Figures ~\ref{fig:master-figure}, ~\ref{fig:code_compose} and ~\ref{fig:code-analysis} to introduce some framework capabilities and familiarize with the Python API. 

\AQ{would remove, will already say in intro} The focus of this work is to explore the ability of AgentTorch to execute million-scale ABMs with LLM-guided agent behavior. In the following sections, we explore the viability of LLM agents for million-scale ABMs and their impact on simulation, calibration, and analysis using AgentTorch. We provide benchmark results and code snippets throughout the paper to demonstrate how LLM agents can be used with AgentTorch to address real-world challenges.

==> content/intro.tex <==
% Code snippets:
% 1. Master figure -> Dynamics + Behavior + Population; get started in 3 lines of code. (Sec 1)

% 2. Sec 3: Gradient-descent; Prompting with archetype 

% 3. Sec 6: Compose with NN for calibration

% 4. Sec 7: Analyze simulation trace for prospective; Debug prompts for counterfactual analysis

% Scalability -> Get started quickly (Sec 1?)
% Differentiability -> Gra; Customize agent (Sec 4)
% Composability -> Compose with NN (Sec 6);
% Flexibility -> Debug prompts (Sec 7); Analyzer (Sec 7)

\section{Introduction}
% Outline of the introduction:
% 1. ABMs are cool - decouple behavior, dynamics and interventions.
% 2. how complexity of dynamics - differentiable ABMs. simple agents.
% 3. how adaptability of behavior - LLM as agents. unrealistic population.
% 4. questions: interaction complexity vs individual agency, how to trade-off?
% 5. contribution: i) benchmark impact on simulation, calibration and analysis; ii) develop framework to unlock real-world utility

% 1. ABMs are cool - decouple behavior, dynamics and interventions.
Many of the today's challenges --- from epidemics to housing shortages to humanitarian crises --- are not the result of a single person's action, but the complex interplay of countless individuals making decisions and interacting over time. Agent-based models (ABMs) aim to capture these dynamics by simulating collections of agents that act and interact within computational environments. ABMs have proven useful across various domains, from evaluating vaccination strategies during the COVID-19 pandemic~\cite{romero2021public, aylett-bullockJuneOpensourceIndividualbased2021b} to predicting the crash of housing markets~\cite{ge2017endogenous, axtell120MillionAgents2016}, and designing evacuation programs for war refugees~\cite{mehrab2024agent,ghaffarian2021agent}.


ABMs have helped study a multitude of complex systems across epidemiology \cite{aylett-bullockJuneOpensourceIndividualbased2021b, kerrCovasimAgentbasedModel2021e, hinchOpenABMCovid19AgentbasedModel2021b}, economics \cite{axtellAgentBasedModeling2022, axtell120MillionAgents2016}, and disaster response~\cite{ghaffarian2021agent,aylett2022epidemiological}. For example, they were used to evaluate vaccination protocols during the COVID-19 pandemic~\cite{romero2021public}, predict the crash of housing markets~\cite{ge2017endogenous}, and design evacuation programs for war refugees~\cite{mehrab2024agent}. ABMs are particularly valuable for addressing these policy questions because they enable the simulation of interventions by modeling the interplay between individual behaviors and environmental dynamics. Their practical utility requires capturing realistic environments and expressive agents while efficiently simulating million-size populations.

% i) disease spread to decide lockdown strategies and prioritize vaccination schedules [], ii) avatars on social networks to understand vaccine hesitancy [], and iii) firms in a financial network to predict housing market crashes []. For example, ABMs have helped inform vaccination protocols during the COVID-19 pandemic [], design evacuation programs for war refugees [] and predict the crash of housing markets []. The emergent behaviors of these complex systems are sensitive to population scale, model specification, and agent behavior. The utility of ABMs for practical decision-making hinges on their ability to capture the complexity of interactions and the adaptability of individual behavior. 

% ABMs are particularly valuable for these policy design questions because they allow for the simulation of interventions by decoupling individual behaviors from environmental dynamics. \AC{talk about importance of scale and adaptability here. P2: Mention advances to capture scale; P3: LLMs cool for behavior but can cause compromise on scale. P4: how to trade-off? need for framework like AgentTorch to balance interaction complexity + individual agency. }

% \AC{state somewhere: ABMs care about macroscopic outcomes, which are sensitive to XYZ.. then we can motivate computational challenges}

%Examples of such complex systems include the spread of epidemics [], supply chain flows [], the housing market [], and many others. Understanding these systems requires modeling techniques that can capture their full complexity, rather than just focusing on modeling a single agent.

%Agent-based modeling (ABM) offers a powerful computational approach for simulating complex systems. In ABM, a system is represented as a collection of autonomous, decision-making entities called agents. The objective is to recreate emergent macroscale properties resulting from the interactions among agents and between agents and their environment.  Consequently, ABMs have been extensively utilized in fields such as epidemiology [], finance [], and biology [], providing insights into phenomena like COVID-19 lockdowns [].

However, the practical application of ABMs has been hindered by two major challenges. First, 
the high computational costs associated with their simulation and calibration processes \cite{bonabeauAgentbasedModelingMethods2002a}. Recent advancements have addressed some of the computational challenges associated with ABMs, enabling the simulation of complex dynamics over millions of agents using vectorized operations 
\cite{chopraDifferentiableAgentbasedEpidemiology2023c, richmondFLAMEGPUFramework2023} and the calibration of models to heterogeneous data sources using differentiable programming~\cite{andelfingerDifferentiableAgentBasedSimulation2023, chopraDifferentiableAgentbasedEpidemiology2023c, montiLearningAgentbasedModels2023b, quera-bofarullBayesianCalibrationDifferentiable2023, tejero-cantero2020sbi, dyerBlackboxBayesianInference2024}. In such differentiable ABMs, deep neural networks also help specify complex environment dynamics~\cite{mordvintsev2020growing}, and autograd helps perform sensitivity analysis --- which evaluates how variations in model inputs affect outputs --- in zero-shot \cite{10.5555/3545946.3598853}. Hence, it is now feasible to simulate, calibrate, and analyze ABMs with millions of agents using commodity hardware. An important remaining limitation, however, is the lack of expressiveness and adaptability of the agents within ABMs.

% These vectorized and differentiable ABMs have also 
% used deep neural networks to specify complex environment dynamics~\cite{neuralnca}; and conduct sensitivity analysis (which evaluates how variations in model inputs affect outputs) using the 

% To address these challenges, deep learning tools have been deployed to enable more efficient and scalable ABM implementations. ABMs' simulation times are sensitive to population scale --- a limitation now mitigated by vectorization across multiple CPUs and GPUs \cite{chopraDifferentiableAgentbasedEpidemiology2023c, richmondFLAMEGPUFramework2023}. ABMs also require the calibration of many free parameters to heterogeneous data sources. This challenge has been addressed by implementing ABM simulators in differentiable and probabilistic programming frameworks \cite{andelfingerDifferentiableAgentBasedSimulation2023, chopraDifferentiableAgentbasedEpidemiology2023c, montiLearningAgentbasedModels2023b, quera-bofarullBayesianCalibrationDifferentiable2023, tejero-cantero2020sbi, dyerBlackboxBayesianInference2024}. Deep neural networks have also been employed to specify complex environment dynamics~\cite{neuralnca}. Sensitivity analysis, which evaluates how variations in model inputs affect outputs, can be performed at zero-shot cost in differentiable ABMs \cite{10.5555/3545946.3598853}. As a result, it is now feasible to simulate, calibrate, and analyze ABMs with millions of agents using commodity hardware. However, these approaches often rely on heuristic agent behavior, limiting their ability to capture the adaptability of individual decision-making.

% An important remaining limitation, however, is the lack of expressiveness and adaptability of the agents within ABMs.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.95\textwidth]{plots/master_figure.png}
%     % \includegraphics[width=0.45\textwidth]{plots/code/agent_torch_sim.png}
%     % \includegraphics[width=0.45\textwidth]{plots/nta_lfpt.png}
%     \caption{(left) Using AgentTorch to simulate disease spread in New York City while capturing adaptive individual behaviors with LLMs (right) Zip-code level employment behavior for 8.4 million agents in NYC estimated using an AgentTorch model calibrated to coarse census data. AgentTorch facilitates modeling collective behaviors emerging from the interplay of individual behavior and environment dynamics, helping overcome limitations of historical data for policy design. \textcolor{red}{Replace left with a pipeline figure + move right to the analysis section - change color map}}
   
%     \label{fig:master-figure}
% \end{figure*}

%Historically, the widespread adoption of ABMs has been hindered by the high computational costs associated with their simulation and calibration processes. However, recent advances in machine learning have addressed these challenges, enabling more efficient and scalable ABM implementations. \AC{instead of leading with the "how", the technical constraints (which are not novel ideas for ML community), lead with the "so what" and then state "how" to show role of ML. Eg: i) ABMs are sensitive to population scale - now solved using vectorized programming. ii) ABMs sensitive to initial conditions and heterogeneous data requirements - solved via differentiable programming; iii) ABM constrained by sensitivity analysis - use gradients help; iv) ABMs also need adaptive behavior - can LLM helps? will need performance trade-offs etc.}

%Firstly, ABM simulators now support vectorization across multiple CPUs and GPUs [], significantly reducing simulation times. Concurrently, developments in differentiable and probabilistic programming have enabled the creation of fully differentiable ABMs []. This facilitates their integration into end-to-end differentiable pipelines, allowing the application of gradient-assisted calibration techniques such as variational inference []. Additionally, amortized neural simulation-based inference techniques have been successfully employed with ABM simulators [], enhancing the accuracy and efficiency of calibration processes. As a result of these advancements, it is now possible to simulate and calibrate ABMs with millions of agents using commodity hardware. Despite this important progress, a remaining pitfall of ABM is its limitation when it comes to agent behaviors that are non-adaptive and non-evolving. For instance, during the COVID-19 pandemic, the response of the public to multiple policies changed across time, as pandemic fatigue and other factors played a role \cite{pangalloUnequalEffectsHealth2024}.

%By leveraging GPU computing and differentiable programming, it is now feasible to calibrate ABMs with millions of agents to real-world data using commodity hardware []. Despite these improvements, ABMs still face limitations due to the restricted expressivity of the constituent agents. In other words, most ABMs assume heuristic rules for agent behaviour which may not be enough to capture the complexity of the real world agents' behaviour. 

% A promising mechanism to overcome this pitfall is the use of generative modeling to design ABM agents. 
Large language models (LLMs) have shown remarkable performance in text-based applications~\cite{openaiGPT4TechnicalReport2024,anilPaLMTechnicalReport2023,touvronLLaMAOpenEfficient2023} which caused a surge in LLM-powered agents with the aim of tackling more general tasks. LLM-as-agents have demonstrated potential to enable more general and adaptive human-like behavior~\cite{serapio-garciaPersonalityTraitsLarge2023,hortonLargeLanguageModels2023}. While promising work on multi-agent simulations with LLM-agents has been performed~\cite{parkGenerativeAgentsInteractive2023,vezhnevetsGenerativeAgentbasedModeling2023a}, it has primarily been limited to tabletop games and small population scenarios. The study of large-scale complex systems, such as epidemics or supply chain networks, often requires the simulation of millions of agents, but little work has been done on scaling LLM-based agent simulations to these numbers. Furthermore, these simulations need also to incorporate adequate environment designs that capture dynamics, such as virus mutations or economic shocks, to be effective for policy design. Our work aims to alleviate this gap. The key question is: How can we leverage the adaptive capabilities of LLMs to enhance agent behavior in ABMs while maintaining computational feasibility for simulations involving millions of agents?

% Large language models (LLMs) such as GPT \cite{openaiGPT4TechnicalReport2024}, PaLM2 \cite{anilPaLMTechnicalReport2023}, and LLaMA \cite{touvronLLaMAOpenEfficient2023}, have demonstrated remarkable performance in text-based applications. This success has caused a surge of research focused on developing LLM-powered agents with the aim of tackling more general tasks. The potential of these agents is supported by studies that have demonstrated LLMs' capability to reproduce different human-like personalities \cite{serapio-garciaPersonalityTraitsLarge2023} and exhibit human-like behaviors across multiple scenarios \cite{hortonLargeLanguageModels2023}. While promising work on multi-agent simulations with LLM-agents has been performed \cite{parkGenerativeAgentsInteractive2023,vezhnevetsGenerativeAgentbasedModeling2023a}, it has been primarily limited to tabletop games and small population scenarios. The study of large-scale complex systems, such as epidemics or supply chain networks, often requires the simulation of millions of agents, but little work has been done on scaling LLM-based agent simulations to these numbers. Furthermore, these simulations need also to incorporate adequate environment designs that capture dynamics, such as virus mutations or economic shocks, in order to be effective for policy design.

\textbf{Summary of Contributions}: The goal of this work is two fold: i) present a mechanism to scale LLM as agents for million-scale ABMs, ii) highlight the nuance between simulation scale and individual agency when using ABMs in the real-world. In this paper, we introduce a mechanism to scale ABMs to millions of agents while integrating LLMs for adaptive agent behavior. First, we validate the viability of LLMs as ABM agents by demonstrating their ability to reproduce census-level statistics of behavior. Next, we introduce the concept of LLM-archetypes representing a collection of agents that share the same behavior characteristics. This approach allows us to scale simulations to millions of agents informed by LLM outputs in an efficient manner. Third, equipped with \AQ{may be overclaim} high-fidelity agents, we analyze the trade-off between simulation scale and expressive individual agents when integrating real-world data. We illustrate our analysis through a case study of 8.4 million agents simulating NYC. Finally, we also present an API to implement and scale LLM Archetype-guided ABM simulations across several domains.

\AQ{this is a bit repetitive with what is above, all of this section should be more concise. I would say: technical contribution: scaling LLM-agents to large populations using archetypes. We then use this technique to study: 1) tradeoff between agency and scale, 2) counterfactual scenarios}
The key contributions are as follows:
\begin{itemize}
    \item Novel use of LLM archetypes: Efficiently scale LLM-based ABM simulations to millions of agents. Section 5 (lines 214-250) demonstrates how LLM archetypes capture realistic population-wide behaviors, validated by Figure 3 which shows correlation with the NYC census data for labor force participation.
    \item Trade-offs between balance between computational efficiency and behavioral nuance. Section 6 (lines 251-293) details the simulation of disease spread and labor market dynamics, comparing different agent architectures (heuristic, archetype, and LLM agents) in forecasting infections and unemployment rates (Figure 4). This showcases our framework's capability to use LLM-prompted behavior in executing and calibrating large-scale ABM simulations.
     \item Capability for retrospective, counterfactual, and prospective analyses: Section 7 (lines 294-327) illustrates downstream benefits for retrospective, counterfactual, and prospective analyses. It demonstrates how adaptive agent behavior can help overcome limitations of historical data in policy design, using examples from the COVID-19 pandemic.
    \item Generic Applicability: We present an API to scale these benefits beyond our current mechanisms and integrated with standard open-source framework for agent-based modeling. More details are provided in the appendix.
\end{itemize}

% \AQ{question: Wasn't agent torch presented last aamas? If so, maybe I would say we use AgentTorch ...} In this paper, we introduce AgentTorch to address these issues. AgentTorch is a framework for scalable simulation, calibration, and analysis of ABMs that allows for the specification of flexible agent architectures and fully differentiable environments. We employ AgentTorch to assess the suitability of LLM agents for large-scale ABM research. First, we study whether LLM-agents can reproduce population-level statistics of behaviour. Next, we introduce the concept of an LLM-archetype representing a collection of agents that share the same behavior characteristics. This approach allows us to scale simulations to millions of agents informed by LLM outputs. Finally, we benchmark the trade-off in simulation fidelity between more expressive individual LLM-agents and a coarser approach based on archetypes. We illustrate our observation through a case study of 8.4 million agents representing NYC.




% All of these points are illustrated through a case study in an epidemiological ABM.
%\cite{mcmillenCollectiveIntelligenceUnifying2024}, such as cells forming organs or animals self-organizing to protect themselves from predators \cite{CollectiveBehaviorSurprisea, camazineSelfOrganizationBiologicalSystems2001}.  Thus it is 

%For example, a decision on the optimal strategy for a vaccination campaign entails considering the characteristics of the virus and the general population, so both individual behaviour and the viral dynamics play an important role.
%\AC{maybe say: a) LLM agents for ABM research - very active but scope is table-top games on small population, ii) challenges - a) current frameworks don't focus on environment design, only agent behavior -> don't scale in population size + not possible to specify mechanistic dynamics which is key for analysis, and policy making, b) how to use LLMs as ABM agents -> not evaluated for "census-plausible" behavior, c) how to scale to million-size populations: balance complexity and agency in simulation?}
%It seems natural, therefore, to consider using LLM agents in the context of ABMs to provide expressive and adaptive agents. While extensive work exists on multi-agent environments with LLM agents, a comprehensive study of their suitability for large-scale simulations is missing. \AC{this seems a bit disconnected to our claims. we need to motivate why large-scale populations. We want don't do anything for i)} Specifically, we ask: i) Can LLMs reproduce the diverse human behaviors relevant to ABM contexts? ii) Can LLM-based ABMs scale to populations of millions of agents? iii) What is the accuracy trade-off between large simulations of simple agents and smaller simulations of more capable agents in reproducing complex systems?

%To address these questions, we introduce the AgentTorch framework: a set of tools for scalable simulation, calibration, and analysis of ABMs with flexible agent architectures. Using the AgentTorch framework, we provide three primary contributions. First, we assess the suitability of LLMs as agents within ABMs by exploring whether a collective of LLMs can replicate observed population behaviors. Second, we introduce the concept of an LLM-archetype, representing a collection of agents that share the same behavior characteristics. This approach allows us to scale simulations to millions of agents informed by LLM outputs. Finally, we benchmark the trade-off in simulation fidelity between using more expressive individual LLM-agents and a coarser approach based on archetypes. These points are illustrated through a case study in an epidemiological ABM.

%Second, we benchmark the trade-off between individual agency and interaction complexity. 

%This paper makes two primary contributions. First, it assesses the suitability of LLMs as agents within ABMs. We explore whether a collective of LLMs can replicate observed population characteristics, respond to environmental changes, and interact with other agents realistically. Second, we benchmark the trade-off between individual agency and collective behavior. Natural systems, such as ant colonies, can self-organize to solve complex problems without relying on highly intelligent individual agents. We aim to study this phenomena through a case study in an epidemiological ABM. \AQ{maybe add stronger contributions, to add later after the conclusions}

%addressing humanity's most significant challenges requires modeling collective behavior. LLMs alone are insufficient for understanding systems where the whole is greater than the sum of its parts. Combining LLMs with ABMs offers promising potential by enhancing ABMs with more expressive, adaptive agents that simulate human-like behaviors more accurately than traditional heuristic-based agents.


%We structure the paper as follows: We begin by outlining related work. Next, we present a case scenario in epidemiology to illustrate example benchmarks. We then introduce the AgentTorch framework, a set of tools for scalable simulation, calibration, and analysis of ABMs with flexible agent architectures. Following this, we describe the experimental setup used to evaluate the trade-off between individual agency and collective behavior, showcasing the generality of our approach with AgentTorch. We then present experimental results, demonstrating the ability of LLM-agents in ABMs to capture complex population behaviors in social settings, with clear instructions for implementation in AgentTorch. Finally, we conclude with our findings and implications.

%\AC{anti-thesis: why not just use langchain?.. importance of the environment in ABMs. Same reason why concordia can't work.}

%Agent-based models (ABMs) aim to capture these dynamics by simulating a collection of agents that act and interact within a computational world. ABMs have been deployed to study a multitude of complex systems including, but not limited to, the housing market [], the spread of epidemics [], the growth of tumors [], and the global supply chain []. This broad applicability is due to their ability to represent decouple heterogeneity of interactions and adaptability of behavior when exploring the emergent effect of dynamics and interventions. \AC{rewrite: relevant since they can decouple dynamics, behavior and intervention}. Practical utility requires recreating populations with detail, capturing adaptive individual behavior and analyzing sensitivity of results.

%For instance, ABMs have helped simulate: i) diseased humans in the physical world to decide lockdown strategies and prioritize vaccination schedules; ii) firms in a financial network to predict housing market crashes; iii) cells in tumor micro-environment to evaluate antibody treatments. 

% 2. complexity of interaction - differentiable ABMs. simple agents.
% 3. agency of individual - LLMs. unrealistic population.
%Emergent outcomes are sensitive to scale of the population, calibration of parameters and, specification of interaction rules and agent behavior. Recent work in differentiable ABMs has helped accelerate simulations of million-size populations, improve calibration to heterogeneous data by integrating with DNNs, learn expressive rule sets via neural model specification and accelerate sensitivity analyzes with gradients. However, these methods have relied on heuristic individual agents. The ability of LLMs to produce plausible individual behavior has opened new possibilities. 



%\textbf{Example}: Consider COVID-19 pandemic where disease dynamics, social mobility and employment considerations were closely coupled together. Years of COVID-19 pandemic demonstrates how human behavior played a key role in shaping these interactions and the consequent effectiveness of interventions. Consider some observations - First, increase in cases prompted conservative mobility behavior by people but people became more carefree when infections decreased. This feedback loop between mobility behavior and disease caused multiple waves. Government imposed lockdowns to artificially constrain mobility behavior but were very harmful for the economy. Second, as time progressed, "pandemic fatigue" kicked in as people lost work, savings dwindled or were emotionally exhausted from caring for family. This influenced ability their compliance to interventions like testing or quarantines, worsening impact on health and economy. Government provided stimulus assistance, child care, mortgage and unemployment assistance to improve compliance to interventions. Which changed characteristics of labor market, creating inflation and hurting industries. Trillions of dollars spend on decision making. Third, trillions of dollars spent on interventions but influenced by behavior - vaccine hesitancy, non-compliance to tests, financial interventions hurt economy. How to allocate resources? Designing disease interventions requires capturing these feedback loops. These dynamics varied significantly across regions and the disease waves. Mitigating the impact of the disease requires capturing these feedback loops. \AC{does this stay here on in problem statement?}

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.4]{plots/astoria3graph.png}
%    \caption{\textbf{Double loop between dynamics and behavior}. \AC{ Placeholder. 3 col of cases, isolation and employment behavior evolving over time. thoughts @arnau?} \AQ{Not sure what this figure shows}. Consider example of disease pandemic. Behavior adapts over time as a result of variation in cases, extrinsic interventions and "pandemic fatigue". Change in mobility and workplace behavior affects dynamics of disease. Agent-based models can help decouple feedback loop between disease, behavior and interventions.}
%    \label{fig:motivation}
%\end{figure}

% Motivate the challenges
%Behavior requires prioritizing individual agency while dynamics requires interaction complexity. The trade-off between individual agency and interaction complexity is tricky to realize. First, can LLM agents even produce "census-plausible" behavior? Populations are sampled from the census, which provides discretized attributes due to privacy and data-availability considerations. Agents are represented with demographic-resolution attributes For instance, "age" is (between 20 to 29), "gender" is (Male), "income" is (90-percentile). Rigorous quantitative analysis for such scenarios is currently missing. Second, how can we leverage such agents when simulating country-scale populations? This is particularly challenging since we the need for online sample of LLM agents at each simulation step. Practically, we would have to either sub-sample the resolution of agency or population.Third, do frameworks exist to design such systems? Current frameworks are inadequate to capture since their either restricted for table-top agent games or small heuristic agents. \AC{need to motivate challenges better: nuances of using LLM as ABM agents? how to design? how to implement?}

% contribution: i) benchmark impact on simulation, calibration and analysis; ii) develop framework to unlock real-world utility
%\textbf{Contribution}: We aim to couple realistic and adaptive individual behavior, with high-resolution population dynamics for simulation, calibration and analysis. This work explores the following questions: are LLM agents via for agent-based modeling? how can we utilize LLM agents for simulating million-size populations? how can we generalize benefits to multiple domains with a generic simulation platform? First, we observe individual behavior can be described in low-dimensional prompts. This enables scaling LLM Agents to million-size populations, by jointly sampling sub-group behavior. Second, we observe such agents can help reparameterize ABMs to decouple behavior and dynamics, resulting in better calibration and counterfactual analysis. Third, we build AgentTorch, a framework to generalize these benefits across multiple domains.

%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=0.8\textwidth]{images/IMG_2195.jpeg}
%    \caption{a) ABMs for population analysis. Current methods have focused on maximizing agency (while studying small populations) or maximizing interconnection (while relying on heuristic agents). What is better? We focus on benchmarking this trade-off. We scale simulations to million-size populations while preserving adaptive individual behavior. b) We also present a framework to build generative populations that scale to millions of agents. AgentTorch provides a simple Python-API to get started in few lines of code. \textcolor{red}{add AgentTorch code snippet}}
%    \label{fig:abm-llm-figure}
%\end{figure}


% Notes:
% Agent-based models (ABMs) aim to capture these dynamic interactions among millions of agents to analyze population level outcomes and have broad relevance across biological, physical, digital and financial realms. For instance, ABMs have helped simulate cells in a tumor micro-environment to evaluate antibody treatments; diseased humans in the physical world to decide lockdown strategies and prioritize vaccination schedules; firms in a financial network to predict housing market crashes. \AC{some transition line? like - practical utility requires recreating the population with great detail, capturing adaptive individual behavior, analysing sensitivity of results?}. Agent-based models (ABMs) [9] are discrete simulators that comprise a collection of agents that can act and interact within a computational world. They represent the heterogeneity of an interacting population via underlying contact networks and model the adaptability of individual agent behavior. This enables domain experts to ground simulations in mechanistic understanding and explore the emergent effects of agent behavior and external interventions. 

% \AC{this paragraph should likely change a lot. Maybe we talk about work in LLM as agents here and highlight the nuance that LLM as agents for ABMs requires?} ABMs can help pursue these challenges by simulating the interplay between dynamics, behavior and interventions. Computationally, constrained by technical challenges for simulation, calibration and analysis of ABMs. AI and ABMs is actively direction of research. Dynamics vary across space and populations, require capturing high complexity. Differentiable ABMs enable simulating million-scale populations, calibrate to heterogeneous real-world data, efficient sensitivity analysis. Used for million-scale policy evaluation during the pandemic. Constrained by how agent expressive behavior is. Behavior adapts with time (multiple waves of analysis) requires high agency. Progress in LLM as agents opens exciting possibilities for capturing adaptive individual behavior. Explored in recent research but constrained to small populations. Also, agents not validated for "census-plausible" behavior. We need methods to merge these two aspects of research.



==> content/notes_expt_setup.tex <==
\section{Environment Design}

We simulate 8.4 million agents representing New York City's population from August 2020 to July 2022, focusing on the interplay between COVID-19 spread and employment dynamics. This period captures multiple disease waves, behavioral adaptations and policy interventions.

\AQ{This section should be much shorter, we just need to introduce the bare minimum, refer to previous paper for details on the models.}
We consider 8.4 million agents that can catch and transmit infections, and be willfully employed. Their state is composed of static (age, gender, income, occupation, household, geo-location) and dynamic attributes (disease status, employment status). The demographic and household characteristics are sampled using the 2022 American community survey (ACS), employment characteristics from the bureau of labor statistics and disease dynamics from the CDC. Agents interact with each other over household, workplace, and mobility networks. We parameterize interactions for recreational and workplace mobility using Google Mobility trends; and household interactions are obtained from the ACS household and migration survey. The census provides summary statistics, which we use to initialize the synthetic populations using standard methods like iterative proportional fitting~\cite{ruschendorf1995convergence}. Hence, we note that the agent population mimics the distribution of New York City, but is not an exact twin (since individual-level microscopic signal is not available).

\textbf{Behavior}: When sampling agent behavior using an LLM, we use GPT-3.5 for all our experiments. The system prompt is provided below:
\begin{tcolorbox}[colback=blue!5!white, colframe=blue!75!black, title=System Prompt]
There is a novel disease. It spreads through contact. It is more dangerous to older people.
People have the option to isolate at home or continue their usual recreational activities outside.
Given this scenario, you must estimate your actions based on
    1) the information you are given,
    2) what you know about the general population with these attributes.

"There isn't enough information" and "It is unclear" are not acceptable answers.
Give a "Yes" or "No" answer, followed by a period. Give one sentence explaining your choice. 
\end{tcolorbox}
We analyze sensitivity to choice of LLM API in the discussion.

\textbf{Environment}: Our experiments focus on the dynamics of disease spread and labor market. We use standard disease~\cite{hinchOpenABMCovid19AgentbasedModel2021b, chopraDifferentiableAgentbasedEpidemiology2023c} and labor models~\cite{li2023large} which have been used extensively in prior work. The disease model capture agent's probability of infection given interaction neighborhood, virus transmissibility ($R_0$) and demographic-specific susceptibility. For disease progression, we follow a standard SEIRM model~\cite{chopraDifferentiableAgentbasedEpidemiology2023c} with discrete transitions at each agent, with generation times obtained from CDC for the delta wave (in progress during December 2020 to April 2021). The labor model captures the unemployment rate based on their individual willingness to work and insured unemployment rates. To make the environment realistic, we capture additional clinical, behavioral and financial interventions - consistent with the protocols in place at that time in the world. For Stimulus Checks, Eligible agents receive stimulus payments at specific time intervals, as was implemented in NYC at the time. Specifically, December 2020 - March 2021 overlaps with the second stimulus check which provided adults \$ 600 and additional \$ 600 for every child. We note that AgentTorch helps differentiate through these stochastic dynamics and also scale the environment to large populations (8.4 million agents).

\textbf{Link between Economic and Epidemiological Models:} The models are coupled through a feedback loop: a) Case numbers affect agents' willingness to work (Sec 4, line 194-200) b) Willingness to work influences labor-force participation rates and workplace interaction networks c) These interaction networks, in turn, affect disease transmission (Equation 8). This coupling is implemented via the LLM prompt (Section 4, line 201). The prompt takes case numbers from the epidemiological model as input and outputs agents' willingness to work. Specifically, In the SIR model (Equation 8), $N_i$ (number of contacts) is influenced by LLM-prompted willingness to isolate and work, which populates mobility and workplace networks respectively. The parameter $\beta$ is calibrated to real-world data. In the labor force model (Equation 9), $W_j(t)$ (willingness to work) is obtained from LLM prompts, while parameters $\gamma_0$ and $\gamma_1$ are calibrated to real-world data. The epidemiological model uses disease transmission dynamics to forecast cases, while the economic model uses labor-force participation rates to forecast unemployment rates. We will enhance Section 6 (lines 258-266) to further clarify this coupling and the interplay between LLM-prompted behaviors and calibrated parameters.

\subsection{Calibration}
\AQ{Move to 6 and way too much details about CalibNN, this is not relevant, could be in preliminaries but not here.}
The goal of this analysis is to demonstrate trade-off between simulation scale and individual agency when calibrating real-world dynamics. We compared three agent agent configurations:
\begin{itemize}
    \item Heuristic: 8.4 million agents with behavior sampled randomly (follows from~\cite{chopraDifferentiableAgentbasedEpidemiology2023c}). This prioritizes simulation scale over agency.
    \item Archetype: 8.4 million agents with 100 LLMs as archetypes. This provides a trade-off between simulation scale and agency.
    \item LLM-Agent: 100 agents with 100 LLMs AS unique per agent (follows from~\cite{parkGenerativeAgentsInteractive2023}). This prioritizes agency over simulation.
\end{itemize}
Archetype samples behavior for each agent based on the variables in the prompt (each simulation agent maps to population archetype). LLM-Agent sub-samples the population, and also re-scales the simulation outputs during calibration.

We conduct calibration with the protocol introduced in~\cite{chopraDifferentiableAgentbasedEpidemiology2023c,quera-bofarullBayesianCalibrationDifferentiable2023,chopra2024framework} where a calibration network (CalibNN) is used to structural parameters and is optimized with gradient from the simulation output. CalibNN is used to predict R0 and IUR for the disease and labor dynamics, respectively and is a GRU (since these parameters are time-varying), as in~\cite{chopraDifferentiableAgentbasedEpidemiology2023c}. Each simulation step is a day for disease dynamics and a month for labor dynamics, consistent with real-world considerations in epidemiology and macroeconomics. For disease model, we aggregate the infection data per week and care with a running average of the CDC case data. For labor model, we compare the unemployment rate estimated at each step with the month-over-month data released by Bureau of labor statistics. We use the MSELoss in both cases. Additional details about the data specification for CalibNN and ground-truth are included in the appendix.

\textbf{Prompt Specification}: The user prompt includes details about individual demographics, time-varying infection statistics, pandemic duration and external interventions. When LLM are used as ABM agents, the prompt inputs are bootstrapped from the simulation. Specifically, we use the case statistics and pandemic duration from the simulation trajectory, instead of ground-truth data. We conduct such "auto-regressive prompting" for two reasons: i) when simulating for prospective interventions, ground-truth data is not available and hence prompt needs to be specified entirely using simulation; ii) when simulation is un-calibrated, the model peaks may not align well with real-world data. In such case, using ground-truth data is unsuitable for capturing the adaptability of behavior (especially when using time-varying information like infections). Hence, since prompt at step $t$ depends upon simulated trajectory at step $t-1$, LLMs need to be sampled online during the simulation. Since behaviors cannot be sampled offline, the trade-off between simulation scale and agent behavior becomes particularly critical. We explored that with the calibration experiment.

Section 4:
We consider NYC with 8.4 million agents. Good to demo large-scale simulation and role of behavior, interventions and environment dynamics in shaping real-world outcomes.
- Motivation
    - COVID-19: Behavior and Environment Feedback (Disease spread and Stimulus)
- Agent
    - Agent Properties
    - Interaction Traces
- Environment
    - Epi Model Equation (Disease spread); Labor Market Equation (Labor Market)
    - Link between Epi and Econ Model
- Behavior
    - Prompt Specification

Section 5: Can archetypes capture richness of agent behavior? [Section 5]
    - Experiment Setup
    - Result
    
Section 6: When calibration to data, trade-off of simulation scale and individual agency? [Section 6]
    - Experiment Setup: (Three Configs: Heuristic, Fully Adaptive and Archetype)
    - Result
    
Section 7: Downstream benefits for counterfactual analysis? [Section 7]
    Pandemic Fatigue and Viral Transmission: What causes destruction? [swap delta and omicron waves?]
    - Sim 1: Model Pandemic Fatigue (Change the Prompt and Observe)
    - Sim 2: Change Environment Dynamics (Observe how that interfaces with Behavior)

Section 8: Discussion
- Analysis of LLM Consistency
- AgentTorch API
- Limitations and Future Scope
    - Going beyond Historical Limits of Data (Retrospective Analysis)

% 3. How does it impact analysis of a simulation?


==> content/notes_motivation.tex <==
\section{Motivation: COVID-19 Pandemic}
\label{sec:motivation}
The COVID-19 pandemic presents a compelling case study for demonstrating the capabilities of AgentTorch and the utility of LLM agents in ABMs. As the pandemic progressed, the complex interplay between disease dynamics, social behavior, and policy interventions posed significant challenges for designing effective public health strategies. The effectiveness of interventions was heavily influenced by human behavior, making it crucial to capture these dynamics in an ABM.

Initially, the feedback loop between mobility behavior and disease spread led to multiple waves of infections, with people adopting more cautious behaviors when cases increased but becoming more relaxed as cases declined~\cite{santana2023covid}. Government-imposed lockdowns aimed at constraining mobility but had severe economic consequences, leading to unprecedented levels of unemployment~\cite{dreger2021lockdowns}. In response, stimulus payments and financial assistance programs were introduced to alleviate economic hardship and encourage compliance with interventions~\cite{li2021impacts}. However, these measures had side effects on the labor market, disrupting employment dynamics and resource allocation for health interventions~\cite{falcettoni2020acts}. As the pandemic continued, "pandemic fatigue" set in, further influencing people's willingness to comply with public health measures like testing, quarantine, and vaccination, exacerbating the impact on health and the economy~\cite{qin2023pandemic}.

To better understand and address these challenges, we focus on two key aspects of individual behavior: isolation and employment. Our goal is to capture how these behaviors vary with: (1) Demographics: age, gender, geo-location, and income status; (2) Disease dynamics: number of new cases in the neighborhood and percentage change from the previous month; (3) Extrinsic interventions: stimulus payments received by the agent to support living expenses; (4) Intrinsic adaptation: duration of the pandemic to capture the effect of "pandemic fatigue" on behavior. We prompt agents for their willingness to isolate and work using the following:

\begin{tcolorbox}[colback=green!5!white, colframe=blue!55!black, title=User Prompt]
You are a \{gender\} of age \{age\}, living in the \{location\} region. You work in \{occupation\} industry with a monthly income of \{income\}. 
\par\vspace{0.1cm}
The number of new cases in your neighborhood is \{cases\}, which is a \{change\}\% change from the previous month. It has been \{duration\} months since the start of the pandemic.
\par\vspace{0.1cm}
This month, you have received a stimulus payment of \{payment\} to support your living expenses.

\par\vspace{0.1cm}
Given these factors, do you choose to isolate at home? (isolation behavior)

\par\vspace{0.1cm}
"There isn't enough information" and "It is unclear" are not acceptable answers.
Give a "Yes" or "No" answer, followed by a period. Give one sentence explaining your choice.
\end{tcolorbox}

The system prompt provides context about the disease dynamics, relative susceptibility of different demographics and is included in Appendix B. We populate the prompts with census-resolution and individual-resolution attributes for LLM-archetypes and LLM-agents respectively. For this paper, we conduct experiments on New York City given its large population and rich social, economic and demographic diversity. We focus on the time horizon from August 2020 to July 2022 since the period characterized by multiple waves of disease, phases of behavioral adaptation, disease evolution, and interventions (see Appendix A for more details on the environment and agent specifications).

With this setup, we benchmark the capabilities of AgentTorch and LLM archetypes through a series of experiments: (1) evaluating the ability of LLMs to recreate population-wide isolation and employment behaviors when prompted with census-based data, (2) comparing the performance of different agent architectures in calibrating to disease waves and unemployment rates, and (3) showcase AgentTorch's utility for retrospective, counterfactual, and prospective analyses of the COVID-19 pandemic. 

% \AQ{would remmove, this will be explained later, we can emphasize it in conclusions} We use AgentTorch to simulate a population of 8.4 million agents representing New York City from August 2020 to July 2022. This period was characterized by multiple waves of disease, phases of behavioral adaptation, disease evolution, and interventions. Our ABM captures the dynamics of disease spread and the labor market while recreating the NYC population with high granularity. (See Appendix A for more details on the environment and agent specifications.). 

\input{content/expt_setup}

